Data driven weak universal consistency

Many current applications in data science need rich model classes to adequately represent the statistics that may be driving the observations. But rich model classes may be too complex to admit estimators that converge to the truth with convergence rates that can be uniformly bounded over the entire collection of probability distributions comprising the model class, i.e. it may be impossible to guarantee uniform consistency of such estimators as the sample size increases. In such cases, it is conventional to settle for estimators with guarantees on convergence rate where the performance can be bounded in a model-dependent way, i.e. pointwise consistent estimators. But this viewpoint has the serious drawback that estimator performance is a function of the unknown model within the model class that is being estimated, and is therefore unknown. Even if an estimator is consistent, how well it is doing at any given time may not be clear, no matter what the sample size of the observations. Departing from the classical uniform/pointwise consistency dichotomy that leads to this impasse, a new analysis framework is explored by studying rich model classes that may only admit pointwise consistency guarantees, yet all the information about the unknown model driving the observations that is needed to gauge estimator accuracy can be inferred from the sample at hand. We expect that this data-derived estimation framework will be broadly applicable to a wide range of estimation problems by providing a methodology to deal with much richer model classes. In this paper we analyze the lossless compression problem in detail in this novel data-derived framework.

==> definitions <==


% packages
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsopn}
%\usepackage{amstex}
\usepackage{latexsym}
\usepackage{graphics}
\usepackage{epsfig}
\usepackage{color}
%\usepackage{epic}
%\usepackage{eepic}
%\usepackage{oldgerm}
% environments
\usepackage{xspace}
\usepackage{tabularx}
%\usepackage{multirow}
\usepackage{wrapfig}

% packages

%\usepackage{amscd}

\usepackage{amsmath} % amsmath stops cases from working
                     % however amsmath contains definition of \text
        
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{array}
\usepackage{color}
\usepackage{epsfig}
%\usepackage{float} % ?
\usepackage{graphics}
\usepackage{latexsym}
%\usepackage{/home/alon/teach/dm/97w/gates/loggates}
%\usepackage{multicol} % ?
%\usepackage{multirow} % ?
\usepackage{pifont}

% to make up for absence of amsmath

\renewcommand{\text}[1]{{\hbox{#1}}}

% definitions

\def \qed     {\Box}  % here because other styles don't use box.


% Blackboard fonts

\newcommand{\EE}{\mathbb{E}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\NN}{\mathbb{N}} % \dN
\newcommand{\QQ}{\mathbb{Q}} % \dQ
\newcommand{\RR}{\mathbb{R}} % \dR
\newcommand{\ZZ}{\mathbb{Z}} % \dZ

% Numbers

\newcommand{\complex}{\CC}
\newcommand{\integers}{\ZZ}
\newcommand{\naturals}{\NN}
\newcommand{\rationals}{\QQ}
\newcommand{\reals}{\RR}
\newcommand{\realsge}{{\reals_{\ge}}}
\newcommand{\realsp}{\reals^+}
\newcommand{\RRp}{\realsp}
\newcommand{\integersp}{{\ZZ^+}}
\newcommand{\integerss}[1]{\ZZ_{\ge{#1}}}

% boldface

\def \ba     {{\bf a}}
\def \bx     {{\bf x}}
\def \by     {{\bf y}}

\def \bA     {{\bf A}}
\def \bB     {{\bf B}}
\def \bC     {{\bf C}}
\def \bD     {{\bf D}}
\def \bF     {{\bf F}}
\def \bG     {{\bf G}}
\def \bL     {{\bf L}}
\def \bQ     {{\bf Q}}
\def \bR     {{\bf R}}
\def \bS     {{\bf S}}
\def \bT     {{\bf T}}
\def \bX     {{\bf X}}
\def \bY     {{\bf Y}}
\def \bZ     {{\bf Z}}

% caligraphics

\def \cA     {{\cal A}}
\def \cB     {{\cal B}}
\def \cC     {{\cal C}}
\def \cD     {{\cal D}}
\def \cF     {{\cal F}}
\def \cG     {{\cal G}}
\def \cH     {{\cal H}}
\def \cI     {{\cal I}}
\def \cK     {{\cal K}}
\def \cL     {{\cal L}}
\def \cM     {{\cal M}}
\def \cN     {{\cal N}}
\def \cO     {{\cal O}}
\def \cP     {{\cal P}}
\def \cQ     {{\cal Q}}
\def \cR     {{\cal R}}
\def \cS     {{\cal S}}
\def \cT     {{\cal T}}
\def \cW     {{\cal W}}
\def \cX     {{\cal X}}
\def \cY     {{\cal Y}}
\def \cZ     {{\cal Z}}

% vectors

\def \vec#1{{\overline{#1}}}

\def \veca  {{\vec a}}
\def \vecb  {{\vec b}}
\def \vecu  {{\vec u}}
\def \vecv  {{\vec v}}
\def \vecV  {{\vec V}}
\def \vecx  {{\vec x}}
\def \vecX  {{\vec X}}
\def \vecy  {{\vec y}}
\def \vecY  {{\vec Y}}
\def \vecz  {{\vec z}}

\def \vct#1{{\overline{#1}}}

\def \vcta  {{\vct a}}
\def \vctb  {{\vct b}}
\def \vctq  {{\vct q}}
\def \vctu  {{\vct u}}
\def \vctv  {{\vct v}}
\def \vctV  {{\vct V}}
\def \vctx  {{\vct x}}
\def \vctX  {{\vct X}}
\def \vcty  {{\vct y}}
\def \vctY  {{\vct Y}}
\def \vctz  {{\vct z}}

\def \vctbeta  {{\vct\beta}}

% Random variables

\newcommand{\rnd}[1]{{\bf #1}}
\newcommand{\rndl}{{\rnd l}}
\newcommand{\rnds}{{\rnd s}}
\newcommand{\rndx}{{\rnd x}}
\newcommand{\rndy}{{\rnd y}}
\newcommand{\rndz}{{\rnd z}}

% arrow vectors

\newcommand{\rvc}{{\overrightarrow c}}

% Abbreviations

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}  % note that overridden in spanish

% notes

%\definecolor{light}{gray}{.75}

\def \mynote#1{{}}

% marginal notes

\def \marcha{{\marginpar{CHNGD}}}
\def \marfix{{\#\marginpar{FIX \#}}}
\def \marnew{{\marginpar{NEW}}}
\def \marok{{\#\marginpar{\# OK?}}}

% qed's

\def \eqed    {\eqno{\qed}}
\def \rqed    {\hbox{}~\hfill~$\qed$}

% sequences

\def \upto  {{,}\ldots{,}}
\def \zn    {0\upto n}
\def \znmo  {0\upto n-1}
\def \znpo  {0\upto n+1}
\def \ztnmo {0\upto 2^n-1}
\def \ok    {1\upto k}
\def \on    {1\upto n}
\def \onmo  {1\upto n-1}
\def \onpo  {1\upto n+1}

% sets

\def \set#1#2{{\{{#1}\upto{#2}\}}}

\def \setpmo   {\{\pm 1\}}
\def \setmpo   {\{-1{,}1\}}
\def \setzo    {\{0{,}1\}}
\def \setzn    {\{\zn\}}
\def \setznmo  {\{\znmo\}}
\def \setztnmo {\{\ztnmo\}}
\def \setok    {\{\ok\}}
\def \seton    {\{\on\}}
\def \setonmo  {\{\onmo\}}
\def \setzon   {\setzo^n}
\def \setzos   {\setzo^*}

\def \sets#1{{\{#1\}}}
\def \Sets#1{{\left\{#1\right\}}}

\def \inseg#1{{[#1]}} % use \intsgm instead
\newcommand{\intsgm}[1]{{[#1]}}

% functions

\def \ord    {\#}

\def \suml   {\sum\limits}
\def \prodl  {\prod\limits}

% Set operations

\def \union  {\cup}
%\def \union  {\bigcup}
\def \unionl {\union\limits}
%\def \Union {\Bigcup} % want this
\def \Union  {\bigcup}
\def \Unionl {\Union\limits}

\def \inter  {\cap}
%\def \inter  {\bigcap}
\def \interl {\inter\limits}
\def \Inter {\Bigcap}
\def \Interl {\Inter\limits}

% Floors and Ceilings

\def \ceil#1{{\lceil{#1}\rceil}}
\def \Ceil#1{{\left\lceil{#1}\right\rceil}}
\def \floor#1{{\lfloor{#1}\rfloor}}
\def \Floor#1{{\left\lfloor{#1}\right\rfloor}}
\def \absvlu#1{{|#1|}}
\def \Absvlu#1{{\left|{#1}\right|}}


% Parentheses, brackets

\def \paren#1{{({#1})}}
\def \Paren#1{{\left({#1}\right)}}
\def \brack#1{{[{#1}]}}
\def \Brack#1{{\left[{#1}\right]}}

%\def \frac#1#2{{{#1}\over{#2}}}
\def \frc#1#2{{\frac{#1}{#2}}}

\def \binomial#1#2{{{#1}\choose{#2}}}

\def \gcd#1#2{{{\rm gcd}\paren{{#1},{#2}}}}
\def \Gcd#1#2{{{\rm gcd}\Paren{{#1},{#2}}}}

\def \lcm#1#2{{{\rm lcm}\paren{{#1},{#2}}}}
\def \Lcm#1#2{{{\rm lcm}\Paren{{#1},{#2}}}}

% number theory

\newcommand{\base}[2]{{[#1]_{#2}}}

% equalities

\newcommand{\ed}{\stackrel{\mathrm{def}}{=}}

\newcommand{\cnvprb}{\stackrel{\mathrm{p}}{\to}}
\newcommand{\cnvdst}{\stackrel{\mathrm{d}}{\to}}
\newcommand{\cas}{\stackrel{\mathrm{a.s.}}{\to}}

%\def \ed     {\,{\buildrel \rm def \over =}\,}
\def \gap    {\ \hbox{\raisebox{-.6ex}{$\stackrel{\textstyle>}{\sim}$}}\ }

\newcommand{\al}[1]{\stackrel{\mathit{{#1}}}{<}}
\newcommand{\ag}[1]{\stackrel{\mathit{{#1}}}{>}}
\newcommand{\ale}[1]{\stackrel{\mathit{{#1}}}{\le}}
\newcommand{\age}[1]{\stackrel{\mathit{{#1}}}{\ge}}
\newcommand{\aeq}[1]{\stackrel{\mathit{{#1}}}{=}}
\newcommand{\ato}[1]{\stackrel{\mathit{{#1}}}{\rightarrow}}

%\newcommand{\eae}{\approx} % exponentially asymptotically eq - replace by \ere
%\newcommand{\eal}{\stackrel<\approx} % replace by \erl

\newcommand{\re}{\sim}
\newcommand{\rle}{\stackrel<\sim} % roughly (asymptotically taken) <=
%\newcommand{\rl}{\stackrel<\sim}
\newcommand{\rge}{\stackrel>\sim}
%\newcommand{\rg}{\stackrel>\sim}

\newcommand{\ere}{\approx} % exponentially roughly equal
\newcommand{\erle}{\stackrel<\approx}
%\newcommand{\erl}{\stackrel<\approx}
\newcommand{\erge}{\stackrel>\approx}
%\newcommand{\erg}{\stackrel>\approx}

% values

\def \half    {{\frac12}}
\def \quarter {{\frac14}}
\def \oo#1{{\frac1{#1}}}

% notation

\def \pr     {{p}}
\def \Pr     {{\hbox{Pr}}}
\def \iff    {{\it iff }}
\def \th     {{\rm th }}

% ignore

\def\ignore#1{}

% Logic

\newcommand{\ra}{\rightarrow}
\def \contra {{\leftrightarrows}}
\newcommand{\ol}[1]{{\overline{#1}}}
%\def \ob {\overline}

\def \ve {{\lor}} % needed?
\def \eq {{\equiv}} % needed?

% spaces

\newcommand{\spcin}{\hspace{1.0in}}
\newcommand{\spchin}{\hspace{.5in}}

% Default text appears in regular print in both book and class versions. 
% There are two types of text that need to be highlighted in class:
% clson - not mentioned in book version (eg jokes)
% clsbk - regular text in book (the parts that need be said)

%For book:
%\newcommand{\clson}[1]{}
%\newcommand{\clsbk}[1]{#1}
%For class:
\newcommand{\clson}[1]{\colorbox{light}{{#1}}}
\newcommand{\clsbk}[1]{\colorbox{light}{{#1}}}

%\newcommand{\bi}{\begin{aopl}}
%\newcommand{\ei}{\end{aopl}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
%\newcommand{\bq}{\begin{quote}}
%\newcommand{\eq}{\end{quote}}

\newenvironment{aopl}
  {\begin{list}{}{\setlength{\itemsep}{4pt plus 2pt minus 2pt}}}
  {\end{list}}

% operators

\def\orpro{\mathop{\mathchoice
   {\vee\kern-.49em\raise.7ex\hbox{$\cdot$}\kern.4em}
   {\vee\kern-.45em\raise.63ex\hbox{$\cdot$}\kern.2em}
   {\vee\kern-.4em\raise.3ex\hbox{$\cdot$}\kern.1em}
   {\vee\kern-.35em\raise2.2ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\andpro{\mathop{\mathchoice
 {\wedge\kern-.46em\lower.69ex\hbox{$\cdot$}\kern.3em}
 {\wedge\kern-.46em\lower.58ex\hbox{$\cdot$}\kern.25em}
 {\wedge\kern-.38em\lower.5ex\hbox{$\cdot$}\kern.1em}
 {\wedge\kern-.3em\lower.5ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\inter{\mathop{\mathchoice
   {\cap}
   {\cap}
   {\cap}
   {\cap}}}
\def\interl {\inter\limits}

\def\carpro{\mathop{\mathchoice
   {\times}
   {\times}
   {\times}
   {\times}}\limits}

\def\simge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}

\def\simle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}

\newcommand{\pfx}{{\prec}}
\newcommand{\pfxeq}{{\preceq}}

\newcommand{\sfx}{{\succ}}
\newcommand{\sfxeq}{{\succeq}}

% for old documents

\newcommand{\twlrm}{\fontsize{12}{14pt}\normalfont\rmfamily}
\newcommand{\tenrm}{\fontsize{10}{12pt}\normalfont\rmfamily}

% picture macros

\newcommand{\grid}[2]{				% grid{width}{height}
  \multiput(0,0)(1,0){#1}{\line(0,1){#2}}
  \put(#1,0){\line(0,1){#2}}
  \multiput(0,0)(0,1){#2}{\line(1,0){#1}}
  \put(0,#2){\line(1,0){#1}}
}

% inductiion macros

%\newcommand{\induction}[3]{
%Inductive statement: {#1}\\
%We prove: {#2}\\
%Basis: {#3}\\
%Step: {#4}\\
%Proof of step: {#5}
%}
\def \Sets#1{{\left\{#1\right\}}}

\def \inseg#1{{[#1]}} % use \intsgm instead
\providecommand{\intsgm}[1]{{[#1]}}

% functions

\def \ord    {\#}

\def \suml   {\sum\limits}
\def \prodl  {\prod\limits}

% Set operations

\def \union  {\cup}
%\def \union  {\bigcup}
\def \unionl {\union\limits}
%\def \Union {\Bigcup} % want this
\def \Union  {\bigcup}
\def \Unionl {\Union\limits}

\def \inter  {\cap}
%\def \inter  {\bigcap}
\def \interl {\inter\limits}
\def \Inter {\Bigcap}
\def \Interl {\Inter\limits}

% Floors and Ceilings

\def \ceil#1{{\lceil{#1}\rceil}}
\def \Ceil#1{{\left\lceil{#1}\right\rceil}}
\def \floor#1{{\lfloor{#1}\rfloor}}
\def \Floor#1{{\left\lfloor{#1}\right\rfloor}}

% Parentheses, brackets

\def \paren#1{{({#1})}}
\def \Paren#1{{\left({#1}\right)}}
\def \brack#1{{[{#1}]}}
\def \Brack#1{{\left[{#1}\right]}}

%\def \frac#1#2{{{#1}\over{#2}}}
\def \frc#1#2{{\frac{#1}{#2}}}

\def \binomial#1#2{{{#1}\choose{#2}}}

\def \gcd#1#2{{{\rm gcd}\paren{{#1},{#2}}}}
\def \Gcd#1#2{{{\rm gcd}\Paren{{#1},{#2}}}}

\def \lcm#1#2{{{\rm lcm}\paren{{#1},{#2}}}}
\def \Lcm#1#2{{{\rm lcm}\Paren{{#1},{#2}}}}

% number theory


% equalities

%\def \ed     {\,{\buildrel \rm def \over =}\,}
\def \gap    {\ \hbox{\raisebox{-.6ex}{$\stackrel{\textstyle>}{\sim}$}}\ }


%\newcommand{\eae}{\approx} % exponentially asymptotically eq - replace by \ere
%\newcommand{\eal}{\stackrel<\approx} % replace by \erl

% values

\def \half    {{\frac12}}
\def \quarter {{\frac14}}
\def \oo#1{{\frac1{#1}}}

% notation

\def \pr     {{p}}
\def \Pr     {{\hbox{Pr}}}
\def \iff    {{\it iff }}
\def \th     {{\rm th }}

% ignore

\def\ignore#1{}

% Logic

\def \contra {{\leftrightarrows}}
%\def \ob {\overline}

\def \ve {{\lor}} % needed?
\def \eq {{\equiv}} % needed?

% spaces


% Default text appears in regular print in both book and class versions. 
% There are two types of text that need to be highlighted in class:
% clson - not mentioned in book version (eg jokes)
% clsbk - regular text in book (the parts that need be said)

%For book:
%\newcommand{\clson}[1]{}
%\newcommand{\clsbk}[1]{#1}
%For class:

%\newcommand{\bi}{\begin{aopl}}
%\newcommand{\ei}{\end{aopl}}

%\newcommand{\bq}{\begin{quote}}
%\newcommand{\eq}{\end{quote}}

% operators

\def\orpro{\mathop{\mathchoice
   {\vee\kern-.49em\raise.7ex\hbox{$\cdot$}\kern.4em}
   {\vee\kern-.45em\raise.63ex\hbox{$\cdot$}\kern.2em}
   {\vee\kern-.4em\raise.3ex\hbox{$\cdot$}\kern.1em}
   {\vee\kern-.35em\raise2.2ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\andpro{\mathop{\mathchoice
 {\wedge\kern-.46em\lower.69ex\hbox{$\cdot$}\kern.3em}
 {\wedge\kern-.46em\lower.58ex\hbox{$\cdot$}\kern.25em}
 {\wedge\kern-.38em\lower.5ex\hbox{$\cdot$}\kern.1em}
 {\wedge\kern-.3em\lower.5ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\inter{\mathop{\mathchoice
   {\cap}
   {\cap}
   {\cap}
   {\cap}}}
\def\interl {\inter\limits}

\def\carpro{\mathop{\mathchoice
   {\times}
   {\times}
   {\times}
   {\times}}\limits}

\def\simge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}

\def\simle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}


% for old documents


% picture macros

% inductiion macros

%\newcommand{\induction}[3]{
%Inductive statement: {#1}\\
%We prove: {#2}\\
%Basis: {#3}\\
%Step: {#4}\\
%Proof of step: {#5}
%}

\usepackage{xspace}
% Rules
% Three letter abbreviation - 
%   first three audible consonants ignoring double letters
%   If < 3 consonants, all consonants and following vowels 
% One or two words: 3-letter abbreviation for each
% Three or more words: first letter from each
% Maintain capitalization, for example \Atn b/c use A

%\newcommand{\aqed}{{\hfill\qed}}  % qed at the end of align - fix!! in glodef

\providecommand{\rndd}{{\bf d}}
\providecommand{\rndx}{{\bf x}}
\providecommand{\rndy}{{\bf y}}
\providecommand{\rndz}{{\bf z}}
\newcommand{\rndT}{{\bf T}}

\newcommand{\cU}{{\cal U}} % moved to glodef
\newcommand{\cV}{{\cal V}} % moved to glodef

\providecommand{\realsge}{{\RR_\ge}}
\renewcommand{\realsge}{{\RR_\ge}}
% Marginal notes

% Later use icons for difficulty. Examples:
% in the clouds, scratching the surface, digging roots, 6 feet under
% Ferrari, Ford, scooter; frazzled, confused, sleepy face,
% number of peppers for difficulty, or \$ for open
% maybe have different ones in different versions of the book

\newcommand{\prbcmt}[1]{{\marginpar{#1}}}
\newcommand{\prbopnqst}{{\prbcmt{Open?}}} % Open problem? (question)
\newcommand{\prbopncrt}{{\prbcmt{Open.}}} % Open problem. (certain)
\newcommand{\prbhrd}{{\prbcmt{Hard.}}} % Hard problem. (certain)
\newcommand{\prbdntknw}{{\prbcmt{Don't know}}} % Don't know.
\newcommand{\prbddnchc}{{\prbcmt{Didn't check}}} % Didn't check.
\newcommand{\cmtchc}{{\prbcmt{Check!}}} % Check 
\newcommand{\chkths}[1]{{\prbcmt{Check!}??? #1 ???}} % Check 
\newcommand{\chcths}[1]{{\prbcmt{!!!}$\Rightarrow$ #1 $\Leftarrow$}} % Check 

\newcommand{\rfrprb}[1]{{Problem~\ref{#1}}} % refer problem
\newcommand{\cer}[2]{{(\ref{#1}.\ref{#2})}} % Chapter + Equation Reference

% Figures

\newcommand{\rsrfgr}[3]{{  % Reserve figure
\begin{figure}[htb]
\begin{center}
\framebox{$#3$ - #1}  % Description inside box
\end{center}   
\caption{#2}   % Caption
\label{#3}     % Label
\end{figure}
}}

% Alphabet

\newcommand{\alphabet}{{\cX}}

% Encodings

\newcommand{\Lss}[2]{{L_{#1}(#2)}}
\newcommand{\Lqvx}{{\Lss q\vctx}}
\newcommand{\elqs}[1]{{\overline L_q(#1)}}
\newcommand{\elpq}{{\overline L_p(q)}}

% Sequential compression

\newcommand{\prbn}{{\prbs n}}

\newcommand{\qrb}{{q}}
\newcommand{\qrbs}[1]{{\qrb^{(#1)}}}
\newcommand{\qrbn}{{\qrbs n}}
\newcommand{\qrbi}{{\qrbs i}}

% Distribution classes

\newcommand{\cPn}{{\cP^n}}

\newcommand{\monotone}{{\cM}}

\newcommand{\Inkss}[2]{{I^{#1}_{#2}}} % iid nk special
\newcommand{\Int}{{\Inkss n2}}      % iid n 2
\newcommand{\Ink}{{\Inkss nk}}      % iid n k
\newcommand{\InP}{{\Inkss n\Ptr}}   % iid n Pattern
\providecommand{\IP}{{I_\Ptr}}      % iid Pattern
\renewcommand{\IP}{{I_\Ptr}}        % iid Pattern
\newcommand{\Iids}[1]{{I_#1}}
\newcommand{\Iidk}{{\Iids k}}
\newcommand{\Iidt}{{\Iids 2}}
\newcommand{\IidZ}{{\Iids\integers}}

% \newcommand{\iidss}[2]{{I^{#1}_{#2}}} % iid nk special % use \Inkss
%\newcommand{\iidnk}{{\iidss nk}}       % iid n k - use \Ink
%\newcommand{\Ik}{{I_k}}                % use \Iidk
%\newcommand{\IZ}{{I_\integers}}        % use \IidZ

\newcommand{\Mnkdsss}[3]{{M^{#1}_{#2,#3}}} % markov n k d special
\newcommand{\Mnkd}{{\Mnkdsss nkd}}         % markov n k d
\newcommand{\Mntd}{{\Mnkdsss n2d}}         % markov n 2 d

%\newcommand{\mrksss}[3]{{M^{#1}_{#2,#3}}} % markov special - use \Mnkdsss
%\newcommand{\mrkntd}{{\mrksss n2d}}       % markov n 2 - use \Mnkd
%\newcommand{\mrknkd}{{\mrksss nkd}}       % markov n k - use \Mntd

% Burrows Wheeler Transform

%\newcommand{\z}{\zeta}  % use \zeta
%\newcommand{\X}{\vecX}   % use \vctX
%\renewcommand{\b}{\beta} % use \beta
\renewcommand{\i}{\iota}  % use \iota
\newcommand{\bs}[1]{b^{#1}}
\newcommand{\bone}{\bs1}
\newcommand{\btwo}{\bs2}

% Markov chain Monte Carlo

\newcommand{\gmc}{G}

% McAllester Schapire

\newcommand{\mmltdltss}[2]{M_{#1}^{#2}}
\newcommand{\mmltdlt}{M_{\mlt}^{\delta}}
\newcommand{\mmltdltt}{M_{\mlt}^{\delta/2}}
\newcommand{\mmltdlttn}{M_{\mlt}^{\delta/{2n}}}

% Fisher information

\newcommand{\score}{y}
\newcommand{\scr}{\score}
\newcommand{\rndscr}{\rnd\score}
\newcommand{\sts}[1]{\score_\theta(#1)}
\newcommand{\stx}{\sts x}
\newcommand{\strx}{\sts\rndx}
\newcommand{\stvrx}{\sts{\vct\rndx}}
\newcommand{\vctscr}{\vct\score} % score
\newcommand{\rvs}{\rnd\vctscr} % rndscr

\newcommand{\scores}[1]{\score_{#1}(x^n)}
\newcommand{\dscores}[1]{\score_{#1}'(x^n)}
\newcommand{\drndscrs}[1]{\score_{#1}'(\rndx^n)}
\newcommand{\ddscores}[1]{\score_{#1}''(x^n)}
\newcommand{\ddrndscrs}[1]{\score_{#1}''(\rndx^n)}

\newcommand{\fshinf}{{J}} % just to check which are I's
\newcommand{\fit}{{\fshinf(\theta)}}

\newcommand{\pps}[1]{{\frac{\partial}{\partial{#1}}}}
\newcommand{\ppt}{{\pps\theta}}

\newcommand{\ppqs}[1]{{\frac{\partial^2}{\partial{#1}^2}}}
\newcommand{\pphs}[1]{{\frac{\partial^3}{\partial{#1}^3}}}

\newcommand{\ppts}[1]{{\pps{\theta_{#1}}}}

\newcommand{\ppvt}{{\pps{\vcttht}}}
\newcommand{\pptt}{{\frac{\partial^2}{\partial\theta_i\partial\theta_j}}}

\newcommand{\wcop}{f^*}
\newcommand{\fml}{\hat{f}}

\newcommand{\ptht}{{p_\theta}}
\newcommand{\ptos}[1]{{\ptht(#1)}}
\newcommand{\ptx}{{\ptos x}}
\newcommand{\ptrx}{{\ptos\rndx}}
\newcommand{\ptvx}{{\ptos\vctx}}
\newcommand{\ptvrx}{{\ptos{\vct\rndx}}}
\newcommand{\ptxi}{{\ptos{x_i}}}

\newcommand{\pvtx}{{p_\vcttht(x)}}


\newcommand{\prbrct}{P_r(\vtr)}
\providecommand{\spr}{{P_r(\theta_r)}}
\newcommand{\vcttht}{{\vct\theta}}     % vector theta
\newcommand{\vtr}{{\vcttht_r}}         % vector theta of rectangle r
\newcommand{\mltx}{{\hat\vcttht(x^n)}} % maximum likelihood theta of x
\newcommand{\mltrx}{{\hat\vcttht(\rndx^n)}} % maximum likelihood theta of rnd x
\newcommand{\rct}{{r}}  % rectangle


% Misc

\newcommand{\vecw}{{\overline \omega}}
\newcommand{\vecp}{{\overline p}}
\renewcommand{\eg}{{\emph{e.g.\ }}}
\newcommand{\iid}{\emph{i.i.d.}\xspace}
\newcommand{\Exp}{{E}}

% Letters

\newcommand{\as}{m}
\newcommand{\mlt}{\mu}
\newcommand{\stype}{\vecu}
\newcommand{\prv}{\varphi}
\newcommand{\prf}{\varphi} % change to \prv (like \mlt)

% Sets

\newcommand{\settnks}[2]{{\cT^{#1}_{#2}}}
\newcommand{\settnk}{\settnks{n}{k}}
\newcommand{\settns}[1]{\cT^{#1}}
\newcommand{\settn}{\settns{n}}
\newcommand{\settsnks}[2]{{\cU^{#1}_{#2}}}
\newcommand{\settsnk}{\settsnks{n}{k}}
\newcommand{\settsns}[1]{\cU^{#1}}
\newcommand{\settsn}{\settsns{n}}

% Compositions

\newcommand{\nop}{{n}}
\newcommand{\Nop}{{\cN}}
\newcommand{\Nopss}[2]{{\Nop^{#1}_{#2}}}
\newcommand{\Nopnk}{\Nopss{n}{k}}
\newcommand{\Nopnm}{\Nopss{n}{m}}
\newcommand{\Nopsss}[3]{{\Nop^{#1}_{#2,#3}}}
\newcommand{\Nopnkm}{{\Nopsss nkm}}

% Ordered partitions

\newcommand{\pop}{{s}}
\newcommand{\Pop}{{\cS}}
\newcommand{\vctpop}{{\vct\pop}}
\newcommand{\Popss}[2]{{\Pop^{#1}_{#2}}}
\newcommand{\Popnk}{{\Popss nk}}
\newcommand{\Popnm}{{\Popss nm}}

\newcommand{\Pops}[1]{{\Pop^{#1}}}
\newcommand{\Popn}{{\Pops{n}}}

% Types

\newcommand{\tpe}{{\tau}}
\newcommand{\tpes}[1]{{\tpe(#1)}}
\newcommand{\tpex}{{\tpe(\vctx)}}

% Scripted vectors

\newcommand{\xss}[2]{{x_{#1}^{#2}}}        % scripted x
\newcommand{\Xss}[2]{{X_{#1}^{#2}}}
\newcommand{\xon}{{\xss1n}}                % x 1 n
\newcommand{\Xon}{{\Xss1n}}
\newcommand{\xomdimo}{{\xss{1-d}{i-1}}} % x -infty to i-1
\newcommand{\xomdomo}{{\xss{1-d}{1-1}}}     % x 1-d to 1-1
\newcommand{\xoimo}{{\xss1{i-1}}}                % x 1 i-1
\newcommand{\xonmo}{{\xss1{n-1}}}                % x 1 n-1

%\newcommand{\xmiz}{{\xss{-\infty}{0}}}     % x -infty to 0
%\newcommand{\xmiimo}{{\xss{-\infty}{i-1}}} % x -infty to i-1
\newcommand{\xmiz}{{\xss{-\infty}{0}}}     % x -infty to i-1
\newcommand{\xmiimo}{{\xss{-\infty}{i-1}}} % x -infty to i-1
\newcommand{\ximdimo}{{\xss{i-d}{i-1}}}    % x i-d to i-1

% Markov 

\newcommand{\order}{d}      % Order
\newcommand{\nc}{{n^c}}     % Number of times state s appeared
\newcommand{\ncx}{{n^{cx}}} % Number of times state s appeared
%\newcommand{\xs}{{x^s}}    % x's following s
\newcommand{\xc}{{x^c}}     % x's following c

\newcommand{\pcs}[1]{p^{#1}}   % probability following c
\newcommand{\pc}{{\pcs c}}     % probability following c
\newcommand{\pcss}[2]{{p^{#1}(#2)}} % probability of x follwing c
\newcommand{\pcixi}{{\pcss{c_i}{x_i}}}   % prob of x's following c_i
\newcommand{\pcxi}{{\pcss{c}{x_i}}}     % prob of x's following c
\newcommand{\pcxc}{{\pcss{c}{\xc}}}     % prob of x's following c

% Context trees

\newcommand{\Td}{{\cP^n_{\settreed}}}
\newcommand{\TSn}{{\cP^n_{\treeS}}}
\newcommand{\Tdn}{{\cP^n_{\treed}}}

\newcommand{\settrees}[1]{{\cT_{#1}}}
\newcommand{\settreed}{{\settrees d}}
\newcommand{\settreeinf}{{\settrees \infty}}

\newcommand{\trees}[1]{{T_{#1}}}

\newcommand{\qctws}[1]{q_{{}_{\textsc{ctw,}#1}}}
\newcommand{\qSs}[1]{q_{{}_{\textsc{#1}}}}

\newcommand{\ternarys}[1]{\tilde{#1}}
\newcommand{\ternaryS}{\ternarys S}

\newcommand{\leaves}{S}

\newcommand{\leavesfbs}[1]{S_{#1}}
\newcommand{\leavesfbd}{{\sets{0,1}^d}}
\newcommand{\leavesfbinf}{\sets{0,1}^\infty}
%\newcommand{\leavesftd}{\ternarys{\leavesfbd}}
%\newcommand{\leavesftinf}{\ternarys{\leavesfbinf}}
\newcommand{\leavesftd}{\tilde{\sets{0,1}}^d}
\newcommand{\leavesftinf}{\tilde{\sets{0,1}}^\infty}

\newcommand{\treeS}{\trees \leaves}
\newcommand{\treeU}{\trees U}
\newcommand{\treeV}{\trees V}
\newcommand{\treebelows}[1]{\trees{*{#1}}}
\newcommand{\treeternaryS}{\trees{\ternaryS}}

\newcommand{\treefbd}{\trees{\leavesfbd}}
\newcommand{\treeftd}{{\trees{\leavesftd}}}
\newcommand{\treefbinf}{\trees{\leavesfbinf}}
\newcommand{\treeftinf}{{\trees{\leavesftinf}}}

% The following are added under the heading distributions:
%\newcommand{\qctwd}{\qctws{d}}
%\newcommand{\qctwinf}{\qctws{\infty}}
%\newcommand{\qS}{\qSs{s}}

% Attenuation

\newcommand{\Atn}{{A}}                % attenuation
%\newcommand{\wrsatn}{{\hat\atn}}     % w-c attenuation - use \Atn

\newcommand{\Aqs}[1]{{\Atn_{#1}}}         % attenuation of q special
%\newcommand{\Atnq}{{\Atnqs q}}            % attenuation of q
%\newcommand{\waq}{{\wrsatn_q}}           % w-c attenuation of q - use \Atnq

\newcommand{\Aqpxsss}[3]{{\Atn_{#1}(#2,#3)}}% attenuation of q for p and x spc
\newcommand{\Aqpx}{{\Aqpxsss qpx}}          % attenuation of q for p and x

\newcommand{\Aqxss}[2]{{\Atn_{#1}(#2)}}   % attenuation of q for x spc
%\newcommand{\aqx}[2]{{\atn_{#1}(#2)}}    % attenuation of q for x - use \Aqxss

\newcommand{\Aqpss}[2]{{\Atn_{#1}(#2)}}   % attenuation of q for p spc
\newcommand{\Aqp}{\Aqpss qp}              % attenuation of q for p
%\newcommand{\waqpss}[2]{{\atn_{#1}(#2)}} % w-c atn of q for p - use \Aqpss
%\newcommand{\waqp}{\waqpss{q}{p}}        % w-c atn of q for p - use \Apq

\newcommand{\AqPss}[2]{{\Atn_{#1}(#2)}}   % attenuation of q for P spc
\newcommand{\AqLPInk}{{\Aqpss{\elp}{\Ink}}} % atn of Laplace for iid nk
%\newcommand{\ApoInk}{{\Aqpss{\elp}{\Ink}}} % atn of Lpl for iid nk -> AqLPInk
\newcommand{\AphInk}{{\AqPss{\ekt}{\Ink}}} % atn of KT for iid nk
\newcommand{\AphInt}{{\AqPss{\ekt}{\Int}}} % atn of Kt for iid n2

\newcommand{\aAqPss}[2]{{\Atn^*_{#1}(#2)}}   % attenuation of q for P spc

%\newcommand{\atnlaplace}{{\waqpss{\qlaplace}{\iidnk}}} % wc atn lpl for iid - use \ApoInk
%\newcommand{\atnktk}{{\waqpss{\qkt}{\iidnk}}}    % wc atn of kt - use \AphInk
%\newcommand{\atnktt}{{\waqpss{\qkt}{\iidss n2}}} % wc atn of kt - use \AphInt

\newcommand{\APs}[1]{{\Atn(#1)}}       % atteuation of P special
\newcommand{\AtnP}{{\APs\cP}}          % worst-case attenuation of P 
\newcommand{\AInkss}[2]{{\APs{\Inkss{#1}{#2}}}} % attenuation of iid special
\newcommand{\AInk}{\AInkss nk}                 % attenuation of iid nk
%\newcommand{\waIss}[2]{{\wrs{\iidss{#1}{#2}}}} % wc atn of iid spc - use \AIss
%\newcommand{\waInk}{{\wrIss nk}}      % w-c atn of iid nk - use \AInk

%\newcommand{\atns}[1]{{\atn(#1)}}     % atteuation of P special - use \APs
%\newcommand{\was}[1]{{\wrsatn(#1)}}   % w-c attenuation special - use \APs
%\newcommand{\atnPs}[1]{{\atn{#1}}}    % attenuation of P special - use \APs
%\newcommand{\waP}[1]{{\wrs{\cP}}}     % w-c atn of P - use \AtnP

\newcommand{\sAqPnsss}[3]{\Atn_#1(#2,#3)} % sqn atn of q for P length n
\newcommand{\sAqPn}{\sAqPnsss q\cP n}

% Redundancy 

\newcommand{\Rdn}{{R}}                % redundancy

\newcommand{\Rqpxsss}[3]{{\Rdn_{#1}(#2,#3)}}% redundancy of q for p and x
\newcommand{\Rqpx}{\Rqpxsss qpx}            % redundancy of q for p and x

\newcommand{\wrsRdn}{{\hat\Rdn}}            % worst-case redundancy
\newcommand{\expRdn}{{\overline\Rdn}}       % expected   redundancy

\newcommand{\wRqpss}[2]{{\wrsRdn_{#1}(#2)}} % w-c redundancy of q for p spc
\newcommand{\wRqp}{\wRqpss qp}              % w-c redundancy of q for p
\newcommand{\eRqpss}[2]{{\expRdn_{#1}(#2)}} % expected rdn of q for p spc
\newcommand{\eRqp}{{\eRqpss qp}}             % expected   redundancy of q for p

\newcommand{\wRq}{{\wrsRdn_q}}        % worst-case redundancy of q
\newcommand{\eRq}{{\expRdn_q}}        % expected redundancy of q

\newcommand{\wRqPss}[2]{{\wrsRdn_{#1}(#2)}} % w-c redundancy of q for P spc
\newcommand{\wRqP}{{\wRqPss q\cP}}  % w-c redundancy of q for P

\newcommand{\wRPs}[1]{{\wrsRdn(#1)}}  % w-c rdn of P special
\newcommand{\wRP}{{\wRPs{\cP}}}       % w-c rdn of P
\newcommand{\eRPs}[1]{{\expRdn(#1)}}  % exp rdn of P special
\newcommand{\eRP}{{\eRPs{\cP}}}       % exp rdn of P

%\newcommand{\wrs}[1]{{\wrsRdn(#1)}}   % use \wRPs
%\newcommand{\wbRs}[1]{{\wrsrdn(#1)}}  % use \wRPs
%\newcommand{\wbRP}{{\wRs{\cP}}}       % use \wRP
%\newcommand{\ebrs}[1]{{\expRdn(#1)}}  % use \eRPs
%\newcommand{\eRs}[1]{{\expRdn(#1)}}   % use \eRPs
%\newcommand{\ebRPs}[1]{{\expRdn(#1)}} % use \eRPs

\newcommand{\wRInkss}[2]{{\wRPs{\Inkss{#1}{#2}}}} % w-c rdn of iid nk spc
\newcommand{\wRInk}{{\wRInkss nk}}              % w-c rdn of iid nk
\newcommand{\wRInt}{{\wRInkss n2}}              % w-c rdn of iid nk

\newcommand{\eRInkss}[2]{{\eRPs{\Inkss{#1}{#2}}}} % exp rdn of iid nk spc
\newcommand{\eRInk}{{\eRInkss nk}}              % exp rdn of iid nk 

%\newcommand{\wbrInk}{{\wRIss nk}} % w-c block red of iid nk
%\newcommand{\wbrIss}[2]{{\wRPs{\iidss{#1}{#2}}}} % use \wRInkss
%\newcommand{\wrIss}[2]{{\wRPs{\Inkss{#1}{#2}}}} % use \wRInkss
%\newcommand{\ebrIss}[2]{{\ars{\iidss{#1}{#2}}}} % use \ebRInkss
%\newcommand{\arIss}[2]{{\ars{\iidss{#1}{#2}}}} % older vrsin of above- change

\newcommand{\wRqMnkdsss}[3]{{\wRqPss q{\Mnkdsss{#1}{#2}{#3}}}} % w-c rdn markov spc
\newcommand{\wRqMntd}{{\wRqMnkdsss n2d}} % w-c rdn of q for markov
\newcommand{\wRMnkdsss}[3]{{\wRPs{\Mnkdsss{#1}{#2}{#3}}}} % w-c rdn markov spc
\newcommand{\wRMntd}{{\wRMnkdsss n2d}}                 % w-c markov

%\newcommand{\wRMsss}[3]{{\wRs{\mrksss{#1}{#2}{#3}}}} % older version - change!
%\newcommand{\wbrMsss}[3]{{\wRs{\mrksss{#1}{#2}{#3}}}} % w-c blk rdn markov spc
%\newcommand{\wRMsss}[3]{{\wRs{\mrksss{#1}{#2}{#3}}}} % older version - change!
%\newcommand{\wbrMntd}{{\wRMsss n2d}} % w-c red of iid nk
%\newcommand{\wRMntd}{{\wRMsss n2d}} % older version of above - change!

\newcommand{\wsRqPnsss}[3]{{\wrsRdn(#1,#2,#3)}} % w-c sqn rdn of q for P lgth n
\newcommand{\wsRqPn}{{\wsRqPnsss q\cP n}}  % w-c sqn rdn of q for P lgth n
\newcommand{\wsRPnss}[2]{{\wrsRdn(#1,#2)}} % w-c sqn rdn of P, length n spc
\newcommand{\wsRPn}{{\wsRPnss \cP n}} % w-c sqn rdn of P, length n spc

%\newcommand{\wsrPqnsss}[3]{{\wRsrdn(#1,#2,#3)}} % use \wsRqPnsss
%\newcommand{\wsrPqn}{{\wsrPqnsss Pqn}} % use \wsRqPn

% Distributions

\newcommand{\dst}[1]{{D(#1)}} % distributions over #1

\newcommand{\pml}{{\hat p}}

\newcommand{\prb}{{p}}
\newcommand{\prbs}[1]{{\prb^{(#1)}}}

\newcommand{\Prb}{\text{Pr}}
\newcommand{\Prbs}[1]{{\Prb^{(#1)}}} % Check if used - phase out

\newcommand{\Prs}[1]{\Pr\Paren{#1}} % phase this out
\newcommand{\Prn}{\text{Pr}} % phase this out

\newcommand{\qctwd}{\qctws{d}}
\newcommand{\qctwinf}{\qctws{\infty}}
\newcommand{\qS}{\qSs{s}}

\newcommand{\pts}[1]{p^{({#1})}}
\newcommand{\ptss}[2]{p^{({#1})}_{#2}}
\newcommand{\pt}{\pts{t}}
\newcommand{\ptpo}{\pts{t+1}}
\newcommand{\ptpoi}{\ptss{t+1}i}
\newcommand{\pti}{\ptss ti}
\newcommand{\pto}{\ptss t1}
\newcommand{\ptt}{\ptss t2}
\newcommand{\ptk}{\ptss tk}

% Estimators 

\newcommand{\est}{{q}}                   % estimator
\newcommand{\eLp}{{\est_{{}_{+1}}}}      % Laplace estimator
\newcommand{\eKT}{{\est_{{}_\textsc{kt}}}}  % KT-estimator
\newcommand{\eEF}{{\est_{{}_\textsc{ef}}}}  % Empirical-frequency estimator
\newcommand{\eGT}{{\est_{{}_\textsc{gt}}}}  % GT-estimator
\newcommand{\eBWT}{{\est_{{}_\textsc{bwt}}}}  % Burrows Wheeler Transform

%\newcommand{\q}{{q}}
%\newcommand{\qlaplace}{{q_{{}_{+1}}}}   % Laplace estimator - use \elp
%\newcommand{\qkt}{{q_{\textsc{kt}}}}    % KT-estimator - use \ekt
%\newcommand{\qef}{{\est_{\textsc{ef}}}} % Emp-frq estimator - use \eef
%\newcommand{\qbwt}{q_{{}_\textsc{BWT}}} % use \ebwt

%\newcommand{\estpo}{{\est_{+1}}}         % use \elp
%\newcommand{\estplshlf}{{\est_{+\half}}} % use \ekt
%\newcommand{\estEF}{{\est_{{}_{\textsc{ef}}}}} % use \eef

% Lempel Ziv 

\newcommand{\lzc}{{\cal L}^{\textsc{lz}}}
\renewcommand{\c}{{c}}

% Patterns

\newcommand{\ptr}{{\psi}}
\newcommand{\vctptr}{{\vct\ptr}}
\newcommand{\ptrs}[1]{{\ptr_{#1}}}  
\newcommand{\ptro}{{\ptrs 1}} 
\newcommand{\ptrt}{{\ptrs 2}} 
\newcommand{\ptri}{{\ptrs{i}}} 
\newcommand{\ptripo}{{\ptrs{i+1}}} 
\newcommand{\ptrn}{{\ptrs n}} 
\newcommand{\ptrnpo}{{\ptrs{n+1}}} 

\newcommand{\ptrss}[2]{{\ptr_{#1}^{#2}}}
\newcommand{\ptroimo}{{\ptrss1{i-1}}} 
\newcommand{\ptroi}{{\ptrss1{i}}} 
\newcommand{\ptron}{{\ptrss1n}}
\newcommand{\ptronpo}{{\ptrss1{n+1}}}
\newcommand{\ptronmo}{{\ptrss1{n-1}}}
\newcommand{\ptroo}{{\ptrss11}}
\newcommand{\ptroz}{{\ptrss10}}

\newcommand{\Ptr}{{\Psi}}
\newcommand{\Ptrs}[1]{{\Ptr^{#1}}}
\newcommand{\Ptrn}{{\Ptrs n}}
\newcommand{\Ptri}{{\Ptrs i}}
\newcommand{\Ptrstr}{{\Ptrs *}}

\newcommand{\ptrof}{\Ptr}
\newcommand{\Xptr}{{\cX^n(\ptr)}}

% Good Turing

\newcommand{\rndmlt}{{\rnd\mu}}
\newcommand{\rndprv}{{\rnd\prv}}
\newcommand{\rndmss}{{\rnd M}}

\newcommand{\train}{{\text{tr}}}
\newcommand{\test}{{\text{ts}}}
\newcommand{\setmlt}{{\cX_\mlt}}
\newcommand{\prvtrns}[1]{{\prv^\train_#1}}
\newcommand{\prvtrnmlt}{{\prvtrns{\mlt}}}
\newcommand{\prbmlt}{{M_\mlt}}
\newcommand{\nmbtst}{{n^\test_\mlt}}

% EM algorithm

\newcommand{\newp}{q}
\newcommand{\bstp}{p'}
\newcommand{\expmltiptrss}[2]{{\tilde\mlt_{#1}(#2)}}
\newcommand{\expmltiptr}{{\expmltiptrss i\vctptr}}

% Continuous

\newcommand{\sqrttpn}{{(\sqrt{2\pi})^n}}
\newcommand{\sqrttpnmo}{{(\sqrt{2\pi})^{n-1}}}
\newcommand{\sqrttp}{{\sqrt{2\pi}}}
\newcommand{\fat}{{\frac\alpha2}}

% Simplex

\newcommand{\smps}[1]{S_{#1}} % Simplex spc
\newcommand{\smpk}{\smps k}   % Simplex k


